SciCap: Generating Captions for Scientific Figures

Researchers use figures to communicate rich, complex information in scientific papers. The captions of these figures are critical to conveying effective messages. However, low-quality figure captions commonly occur in scientific articles and may decrease understanding. In this paper, we propose an end-to-end neural framework to automatically generate informative, high-quality captions for scientific figures. To this end, we introduce SCICAP, a large-scale figure-caption dataset based on computer science arXiv papers published between 2010 and 2020. After pre-processing - including figure-type classification, sub-figure identification, text normalization, and caption text selection - SCICAP contained more than two million figures extracted from over 290,000 papers. We then established baseline models that caption graph plots, the dominant (19.2%) figure type. The experimental results showed both opportunities and steep challenges of generating captions for scientific figures.

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/abstract.tex <==



%edited by MB
Researchers use figures to communicate rich, complex information in scientific papers.
The captions of these figures are critical to conveying effective messages. 
However, low-quality figure captions commonly occur in scientific articles and may decrease understanding.
In this paper, we propose an end-to-end neural framework to automatically generate informative, high-quality captions for scientific figures.
%When researchers write papers, a neural-caption model trained on captions can be used to suggest useful captions.
To this end, we introduce \textbf{\dataset},\footnote{\dataset is available at: \url{https://github.com/tingyaohsu/SciCap}} a large-scale figure-caption dataset based on computer science arXiv papers published between 2010 and 2020.
After pre-processing -- including figure-type classification, sub-figure identification, text normalization, and caption text selection -- \dataset contained more than two million figures extracted from over 290,000 papers.
We then established baseline models that caption graph plots, the dominant (19.2\%) figure type.
The experimental results 
%We also established several image-captioning baselines, 
showed both opportunities and steep challenges of generating captions for scientific figures.

%We establish several strong baselines for the storytelling task, and
%motivate an automatic metric to benchmark
%progress.

%Experiments showed that the proposed framework produces better captions than other baselines\kenneth{THIS IS NOT TRUE}, shedding light on the possibilities of future automatic writing support options for figure captions.

%-------------- dead kitten -------------

\begin{comment}
% \kenneth{UPDATE NUMBERS ACCORDINGLY}
% Kenneth: I did a sentence-by-sentence re-write based on your text. Try to use simple, direct, short sentences in your future writing.

% Figures contain rich and useful information that is human friendly to read due to the inherency of visual format. In certain formats, such as graph plots, bar charts, tables, especially in scientific fields have been widely using to help people better understand the data representation. 
Researchers use figures to communicate rich and complex information in scientific papers.
%
% People also use machines to process those data efficiently. --> I removed this one. It's not relevant to your core argument.
%
% Although figures are straightforward for humans to read, sometimes it could be confused for non-domain experts or people who are working outside this specific field to realize the core concept of the figures. And further, lots of descriptive captions of those figures are ambiguous and do not provide any detailed information. 
The captions of these figures are critical to convey the messages effectively.
%
% Not to mention that it is even harder for machines to process them. --> Removed again. "Help computer" is NOT your core motivation.
%
% In the paper, we propose a novel end-to-end framework to automatically generate captions for scientific figures. --> Don't jump to "what you do". You will need a "HOWEVER" first.
However, low-quality figure captions %(such as \textit{``Results of Experiment 1''}) 
occur commonly in scientific articles, which do not help, or even hurt, understanding. %This is the HOWEVER.
In this paper, we propose to use an end-to-end neural framework to generate captions for scientific figures automatically. %This is the solution for the HOWEVER.
When researchers write papers, a neural caption model trained on informative, high-quality captions can be used to suggest useful captions.%Say more about WHY it's the solution for the HOWEVER.
%
% We first collect the recent real-world scientific papers (from 2010 - present), especially in flourishing computer science fields. 
To this end, we introduce \textbf{\dataset}, a large-scale figure caption dataset based on arXiv papers in Computer Science published between 2010 to 2020.
% Then we parse the figures via several steps such as localization, classification, and analysis of each component of the figures.
After pre-processing --- including figure type classification, sub-figure identification, text normalization, and caption text selection --- \dataset contains more than two million figures were extracted from over 290,000 papers.
% We focus on graph plots which is the most dominant and clear defined category of scientific figures. We further develop neural image caption models that generate high-quality captions for those figures.
We then develop image captioning models for graph plots, which is the dominant (19.2\%) figure type.
% Experiments show that our proposed framework can generate reasonable captions for scientific figures under several metrics and outperforms the baselines in human aspects, thus claiming a significant potential for the automatic detailed captioning of scientific figures.
Experiments show that the proposed framework produce better captions than other baselines, shedding lights on the possibilities of future automatic writing supports for figure captions.



\end{comment}


==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/baselines.tex <==
We use CNN + Long short-term memory(LSTM) structure as our baseline, which is typical architecture in Image Captioning task~\cite{xu2015show}. We extract the images features using the pre-trained  ResNet-101 model~\cite{he2016deep} and represent each figure a 2048-dimensional  vector. We then feed the vector into a dense layer to fit the dimension of word embedding and learn the adjusting transformation. 

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/conclusion.tex <==
%edited by MB
This paper introduces \dataset, a large-scale image-captioning dataset that contains real-world scientific figures and captions. 
%\dataset was constructed using the papers collected and released by arXiv, containing more than two million figures were extracted from over 290,000 papers.
\dataset was constructed using more than two million images from over 290,000 papers collected and released by arXiv.
We also established	several image-captioning baselines, showing the feasibility and challenges of generating captions for scientific figures.
In the future, we will explore approaches to improve caption quality, such as taking advantage of large pre-trained language models~\cite{Beltagy2019SciBERT}, %in specific domains, 
or using information in paper's full text to boost performance.
%or learning to post-edit the generated captions~\cite{hsu-etal-2019-visual}.

%\kenneth{Say slightly more about using the paper}
%\kenneth{One of the future direction can also be post-editing. Cite our own paper.}

%------------- dead kitten ----------

\begin{comment}



% \kenneth{UPDATE NUMBERS ACCORDINGLY}
This paper introduces \dataset, a large-scale image captioning data that contains real-world scientific figures and captions.
\dataset was constructed using the papers collected and released by arXiv,
%\dataset 
containing more than two million figures were extracted from over 290,000 papers.
% We focus on graph plots which is the most dominant and clear defined category of scientific figures. We further develop neural image caption models that generate high-quality captions for those figures.
We also establish several image captioning baselines, showing the feasibility and challenges of generating captions for scientific figures.

In the future, we will explore novel approaches to improve the caption quality.
For example, taking advantage of large pre-trained language model in specific domain, or use the extra information in the paper, to boost the performance.


\end{comment}

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/data.tex <==

%\kenneth{The size of data in each step is important. Make sure you keep track of all of them.}\edward{correct}


%edited by MB
%Most prior work used synthesized data to train figure-captioning models.
%Real-world figures and captions, on the other hand, are much richer and also much nosier.\kenneth{noisier is not so easy to understand.}\edward{contain more diverse and details information}
This section describes the process that massages real-world figure-caption data into an appropriate easy-to-use format for the NLP community.
This data-processing procedure was developed iteratively and empirically.






%edited by MB
\paragraph{Step 1: Data Acquisition and Pre-processing.}
Data acquisition is a fundamental challenge for constructing a public scientific figure-caption dataset.
Although there is a vast number of scientific papers, they are not all easy to access.
\dataset is based on the arXiv dataset~\cite{clement2019arxiv}.\footnote{arXiv Dataset on Kaggle: \url{https://www.kaggle.com/Cornell-University/arxiv}}
%\cy{Is it from this paper ``ON THE USE OF ARXIV AS A DATASET''?}\edward{yes, and Kaggle found it}\cy{Cite it as well then}\edward{\cite{clement2019arxiv}}
The arXiv dataset is licensed under CC-0, which grants remake and republish rights.
It contains a repository of 1.7 million articles with relevant features, such as article titles, authors, categories, abstracts, full-text PDFs, and more.



%edited by MB
We first downloaded all the scholarly articles from the arXiv dataset and froze the date on Dec 22, 2020 (a total of 1,921,287 papers). 
\dataset does not include any papers published after this date.
We further narrowed our dataset to papers published between 2010 and 2020 in computer science (cs.) and machine learning (stat.ML) topics, which numbered 295,028 papers.
%\kenneth{make sure the number is correct}\edward{correct}
We did not use these papers' ``source files,'' which might contain the original LaTeX and figure files. Not all papers come with source files; some source files have complex dependencies that are hard to parse.
%\cy{Change the following paragraph?}
%Note that we did not use the papers' source files, which might include the original LaTeX files and figure files.
%We did not use these source files because not all papers have source files. 
%Some paper's source files even have complex dependencies that are not easy to parse.
%\cy{Although source files might contain the original LaTeX and figure files,
%not all papers come with the source files and these source files might have complex dependencies that are hard to parse.}




%edited by MB
\paragraph{Step 2: Figure-Caption Pair Extraction.}
We then used PDFFigures 2.0~\cite{clark2016pdffigures} to extract the figures from papers in our paper collection.
PDFFigures 2.0 is a Scala-based tool created to extract figures, captions, tables, and section titles from scholarly documents, with a focus on
% documents from the domain of computer science.
the computer science domain.
%edited by MB
In addition to the figures' images and captions, the tool also extracted all
%the exact coordinates of those components\kenneth{What components exactly?} \edward{they give every figure and text coordinates of region in the paper}and 
the text snippets inside the figures, such as legends, X-Y labels, and titles.
%\kenneth{What exactly is the text snippets? Title? Legend?}\edward{any text inside the figure, legend, x-y labels, title if in figure}
%Potentially, 
The extracted information can be used to boost the performance of image-captioning models.
%\kenneth{We can remove this to save space if needed.}
This step resulted in 295,028 papers and 2,170,719 figures.


%edited by MB
\paragraph{Step 3: Figure Type Classification.}
Given the high diversity in the figure types included in scientific articles, we did not aim to create a single captioning model for all types of figures.
Instead, we aimed to create captioning models specialized for one particular figure type.
%From a writing support perspective, the author of the paper  
%\kenneth{Add some writer scenarios maybe?}
We used an automatic figure type classifier~\cite{siegel2016figureseer} to classify	figure type in \dataset.
This pre-trained classifier	can identify seven types of figures: 
graph plots,
flowcharts (also called node diagrams), 
equations (also called algorithms), 
bar plots, 
scatter plots, 
tables, 
and ``other.''
Its reported accuracy is 86\% over 60,000 samples~\cite{siegel2016figureseer}.	



%edited by MB
According to the classifier's prediction, out of 2,170,719 figures, 
19.2\% (416,804) are graph plots,
23.6\% (511,984) are tables,\footnote{In this work, tables are not considered to be figures due to drastically different visual features and contents.}
5.9\% (127,197) are	equations (including algorithms and pseudo codes),
8.5\% (185,398) are flowcharts, 
2.0\% (44,052) are scatter plots, 
4.7\% (101,146) are bar charts, and	
36.1\% (784,138) are ``other.''
In \dataset, we only focus on graph plots, which have the highest classification performance~\cite{siegel2016figureseer} and are also the most common figure type.
%()
% Due to drastically different visual features, content, and uses, we did not consider tables to be figures.
% \cy{Do you ``only'' consider ``graph plots''? or only ``tables'' are removed?} \edward{only consider graph plots}




%edited by MB
\paragraph{Step 4: Removing Figures with Subfigures.}
%Real-world data is rich but noisy; the quality, length, and amount of information varies significantly among captions in published papers.
Many scientific figures contain subfigures.
For example, in our pilot study	(Section~\ref{sec:2000-figure-study}), 35.72\% of overall scientific figures had subfigures.
\dataset focuses on generating captions for single figures, so we removed figures with %more than one 
subfigures from the dataset.
We first used handcrafted rules to identify captions that explicitly mention or refer to subfigures [for
example, \texttt{(a)}, \texttt{a)}, \texttt{(b)}, \texttt{b)}, \texttt{(1)}, \texttt{1)}, \texttt{(2)}, \texttt{2)} ... etc.]. 
%This rule-based approach yielded high classification precision but low recall.
%(See Section~\ref{sec:2000-figure-study}).
%\kenneth{Are these numbers based on the 2000 images you labeled?}\edward{yeap}
%To increase the recall, 
Furthermore, we also used FigureSeparator~\cite{tsutsui2017data} to filter figures with subfigures out of our collection.
FigureSeparator is a CNN-based model 
that separates compound figures in the ImageCLEF Medical dataset with 85.9\% accuracy.

%that separates compound figures with 85.9\% accuracy on the ImageCLEF Medical dataset. 
Of 416,804 graph plots identified in Step 3, the rule-based approach yielded
%first removed images with subfigures and kept
352,719 graph plots, and the FigureSeparator further narrowed the collection down to 133,543 figures.
%Namely,
An estimated 32.04\% of the graph plots did not have subfigures.
%were passed to the next step.
%416,804 啥都沒做的graphplot
%rule-based之後3522719
%rule-based+separator之後 133543
%416,804 * 32.04% = 133543
%416,804 * 67.96% = 283261
%Of 133,543 graph plots identified in the previous step, 67.96\% contained subfigures, which we removed from our dataset.
%\kenneth{CHECK NUMBER. This number is still incorrect. ``Of 133,543 graph plots identified in the previous step'', but in Step 3 we said ``416,804'' graph plot}
%\edward{32.04\% are single figure, 67.96\% are multiple figures}
%\kenneth{Q for Ed: If this is the case, WHY in Section~\ref{sec:2000-figure-study} only 35.72\% of figures DID HAVE subfigures? Because Graph Plot has more subfig??? }


%edited by MB
\paragraph{Step 5: Text Normalization.}
%In \dataset, 
We used NLTK~\cite{Loper02nltk:the} for tokenization and converted all the text to lowercase.
We also removed the figure numbers, such as ``Figure 1:'' or ``Fig. 1:'', and only kept the main caption text.
%and then applied 
The following two text normalization strategies were then applied:

%\vspace{-.4pc}

\begin{itemize}
    
    
%edited by MB
\item \textbf{Basic Normalization:}
We replaced all the numbers ({\em e.g.}, \texttt{0}, \texttt{-0.2}, \texttt{3.44\%}, \texttt{1,000,000}) with \texttt{[NUM]}.
%\kenneth{Did I miss any thing? Negative sign, percentage, interger...}
%We also removed all instances of the percentage sign (\%).
%\kenneth{What does this sentence mean? removed all instances of the percentage?}
%\kenneth{Q for Ed: Did you do the tokenization and lowercase for the first raw in the experiments? I thought you at least need to do lowercase?...}\edward{yes, I also do naive normalization that tokenize, lowercase and remove the initial title (e.g. Figure x./fig. x.)}

%\vspace{-.5pc}

%edited by MB
\item \textbf{Advanced Normalization:}
%We further performed advanced normalization operations.
We created regular expressions
%We adapted the regular expressions used in ARQMat~\cite{mansouri2020finding}, which was created to recognize equations in LaTeX codes, 
%which is powered by a rich set of regular expressions, 
to identify equations in captions and replaced them with \texttt{[EQUATION]}.
%\kenneth{Do we really need to cite ARQMat? Ed, if we just use some heuristics to find equations, %we might not need to cite ARQMat.}\edward{you may remove it}
%\kenneth{How exactly did you adapt their regular expressions? Example?}\edward{simple way, if [words] = [NUM]}
We also replaced all the text spans enclosed by any types of bracket pairs, including \texttt{\{\}}, \texttt{[]}, and \texttt{()}, with \texttt{[BRACKET]}.

%\kenneth{ADD explanation about it can be improved.} \kenneth{Add examples why it worked?} \edward{Since the regular expression method used in \cite{mansouri2020finding} is used in latex format contains special symbols which is easier and more accuarate to recognize the range of math equation compare to pure text. Other methods could be either train a model to label math equation in text or use image recognition of math equation purposedd by \cite{mali2020scanssd}} 
%\kenneth{Give me (1) some example regular expressions and (2) some before/after captions here.}

\end{itemize}

%\vspace{-.7pc}

%edited by MB
\paragraph{Step 6: Target Caption Text Selection.}
\dataset provides three different data collections, each sampled using different strategies:

%\kenneth{We also calculated the percentage of one-sentence captions and the average length of a caption:}\edward{do you want avg sentences/tokens}
%[Data Cleaning Method: % of caption w/ one sentence, Avg. #sentence per caption]
%Original: 59.42%, 1.87
%Rule-Based: 63.98%, 1.70
%Rule-Based+FigureSeparator: 70.47%, 1.51

%\vspace{-.5pc}

\begin{itemize}


    
%edited by MB
\item \textbf{First Sentence (133,543 Figures):} 
This collection includes all the figures.
For each figure included, this collection only includes the first sentence of the caption.
%
%\vspace{-.5pc}


%edited by MB
\item \textbf{Single-Sentence Caption (94,110 Figures):} 
This collection includes the complete caption of only the figures with a one-sentence caption.
%Namely,  
Of the graph plots, 70.47\% had a one-sentence caption.
%Note that this collection is a subset of the First Sentence collection.
%\kenneth{ADD NUMBER HERE, 94110/133543 = 70.47 maybe?}
%\vspace{-.5pc}

 
%edited by MB
\item \textbf{Caption with No More than 100 Words (131,319 Figures):} 
This collection includes the complete caption of only the figures %with a one-sentence caption. 
%This collection includes only the figures 
whose captions contained no more than one hundred tokens (punctuation marks included).
In this collection, a caption contains 1.66 sentences on average (SD=1.07).
%\kenneth{ADD NUMBER!!!}\edward{done}
%\kenneth{Does 100 tokens include punctuation marks (?!.,)?} \edward{yes}
%'s first sentence had no more than 100 to- kens.
%For each figure included, this collection includes the maximum number of sentences (counted from the beginning of the caption) be- fore exceeding 100 tokens.
 
 
\end{itemize}

%\vspace{-.5pc}

On average, with advanced normalization (Step 4),
a sentence in the ``First Sentence'' collection contains 23.19 tokens (SD=20.86);
a sentence in the ``Single-Sentence Caption'' collection contains 14.05 tokens (SD=8.15);
and a sentence in the ``Caption with No More Than 100 Words'' collection contains 22.04 tokens (SD=17.44).
%\kenneth{Oh, so the ``First Sentence'' collection is NOT shorter than ``Caption with No More Than 100 Words'' collection? Because some of the first sentences are super long?}\edward{I think is longer? In the advanced setting, yes. There indeed some cases first sentence super long, I can find some examples if needed.}
%\kenneth{Typo, I missed the ``NOT'': Is the ``First Sentence'' collection NOT shorter???}\edward{Let me parse to see}
%\kenneth{ADD NUMBERS HERE!!!}\edward{done}
%\kenneth{TODO: Add SD}\edward{done}



%Training, validation, and test sets 
Note that we first created the 80/10/10 train/val/test data split for the entire corpus and then proceeded with the caption selection step.
This procedure ensured that we used the identical set of figures to construct each collection's test set; the
same applied to their training and validation sets.
%For example, if the First Sentence collection's test set contains a figure with a ten-word single-sentence caption,
%the same figure occurs in the test sets of the other two collections, too. \kenneth{This FOR EXAMPLE feels quite extra...}


%For example:

%+Figure X’s caption has 1 sentence. Figure X is included in the test set of (a), (b), and (c). (a) and (b) uses the whole one sentence; (c) uses the first 100 words.
%+Figure Y’s caption has 2 sentences. Figure Y is included in the training set of (a) and (c). (a) uses the first sentence; (c) uses the first 100 words. (b) doesn’t select this figure because it only selects captions with a single sentence.

%So, if the Text Data is different, the figures in the test/dev/train splits are roughly the same, but the caption texts are different. 




%Despite all the data processing and filtering strategies applied in the previous steps, the remaining figures still had quite a diverse range of caption types. 

%\input{tech-eval-table}

\input{tech-eval-table-graph-plot-only}

\subsection{Data Analysis and Quality Measurement}
\label{sec:2000-figure-study}


%edited by MB
To evaluate the quality of our data cleaning and processing pipeline, we randomly sampled 2,000 figures from the original arXiv dataset, and one author manually labelled each figure's figure type and whether it contained subfigures (Yes/No).\footnote{To validate the label quality, we had three graduate students label 100 figures, respectively.
On average, they %three annotators 
agreed with 97\% of our subfigure labels.
%\kenneth{TODO: Use Ed's subfig (Y/N) labels as gold-standard label and calculate each of their accuracy (?/100) and then average the accuracy.}\edward{done}
For the figures without subfigures, they agreed with our figure type labels 82.17\% of the time.
%\kenneth{TODO: Similarly, calculate their average accuracy}\edward{done}
For the figures with subfigures, they agreed with at least one of our type labels 86.56\% of the time.
%\kenneth{TODO: You can probably use hand to count numbers here. We only have like around 30 figures with subfigures?}\edward{done}
}
Of these 2,000 figures, 1,926 figures had no extraction errors, and were included in our follow-up calculation.
%\kenneth{Do we have anything like Kappa here?}\edward{what does that mean?}\kenneth{Did you compare Hua/CY/Chacha's labels with yours, or with each other, in any ways? Could we say something here?}
%\kenneth{How exactly you label the data? Each figure was annotated by one or two person?}\edward{I create interface and annotated 2000 samples myself}\kenneth{Wait I thought CY Chacha and Hua helped???}\edward{they just do cross validation for 100 examples, nobody would like to annotate 2000 sample except me}
%\kenneth{Explicitly talk about multi-type subfigures. --> We annotate multi class since this is more realistic.}
As for types, 20.35\% of the figures were graph plots, 4.1\% were bar charts, and 3.11\% were scatter plots.\footnote{A figure might contain subfigures of different types ({\em e.g.}, a bar chart accompanied by a graph plot.) For each figure, we took a multi-class labeling strategy that exhaustively labels all distinct types of its subfigures.}
%\kenneth{This is the FIGURE type, correct?}\edward{correct}
%\kenneth{We might want to explain complex relations between subfigs and types.}
In terms of subfigures, 237 out of 1,926 figures (35.72\%) contained subfigures:
33.14\% of these figures contained graph plots as subfigures,
5.81\% contained bar charts, and 
6.83\% contained scatter plots.

%\kenneth{Since we used multi-class labels, the word ``contained'' is probably more accurate than `` were''?}\edward{okay}
%\kenneth{TODO: Do we consider subfig here?}\edward{what does that mean?}



%edited by MB

We used these 1,926 labeled images to evaluate the tools we employed in constructing \dataset.
Table~\ref{tab:tech-eval} shows the results.
For the figure type classification, the overall performance over graph plots were reliable.
Regarding identifying the graph plots (as labeled automatically in Step 3) that do not contain subfigures, FigureSeparator had an exceptionally high precision.
%the rule-based classifier yielded high precision but low recall, and adding FigureSeparator improved overall performance.\kenneth{This whole sentence needs update}





%-------------- dead kitten -------------

\begin{comment}


\kenneth{--------------------- the following becomes Table 1 ------------}


%edited by MB
\paragraph{Figure Type Classifier.}
The overall performance over graph plots and bar charts type was reliable.\kenneth{OR say it's close to what was reported.}
For the graph plots, Accuracy = 0.95, Precision = 0.9, Recall = 0.83, F1-Score = 0.87. 
For the bar	charts, Accuracy = 0.99, Precision = 0.85, Recall =	0.78, F1-Score = 0.81.




%edited by MB
\paragraph{Rule-Based Subfigure Classifier.}
As	mentioned, the rule-based subfigure classifier yielded high classification precision (0.82 in graph plots; 0.71 in bar charts) but low recall (0.36 in graph plots; 0.17 in bar charts).


%edited by MB
\paragraph{FigureSeparator Subfigure Classifier.}
The	overall performance of FigureSeparator in graph plots was reliable:  
Accuracy = 0.82, Precision = 0.7, Recall = 1.0, F1-score = 0.82.
\kenneth{Is this AFTER rule-based, or are separate from rule-based's results?}

\paragraph{FigureSeparator Subfigure Classifier.}
The overall performance of FigureSeparator in graph plots are reliable: Accuracy = 0.82, Precision = 0.7, Recall = 1.0, F1-score = 0.82.


\paragraph{Rule-Based Subfigure Classifier.}
As mentioned, the rule-based subfigure classifier yields a high classification precision (0.82 in graph plots, 0.71 in bar charts) but a low recall (0.36 in graph plots, 0.17 in bar charts).


\paragraph{Figure Type Classifier.}
The overall performance over graph plots and bar charts type are reliable. For the graph plots, Accuracy = 0.95, Precision = 0.9, Recall = 0.83, F1-Score = 0.87. For the bar charts, Accuracy = 0.99, Precision = 0.85, Recall = 0.78, F1-Score = 0.81. 

We also use these 1,926 labeled images to evaluate the tools we employ in constructing \dataset:

\kenneth{This is where we talk about the data that produced at the end of Step 6}
To evaluate the quality of our data cleaning and processing pipeline, we randomly sample 2,000 figures from the original arXiv dataset and manually label each figure's figure type and subfigures (Yes/No).
Among these 2000 figures, 1,926 figures have no extraction errors and are included in our follow-up calculation.
%\paragraph{Data Analysis.}
As for types, 20.35\% of the figures are graph plots, 4.1\% are bar charts, and 3.11\% are scatter plots.
As for subfigures, 688 out of 1,926 figures (35.72\%) contain subfigures: 33.14\% of these figures are graph plot,
5.81\% are bar charts, and
6.83\% are scatter plots.
%mention the 20000 subfigure stats.

 \item \textbf{First 100 Words (131,319 figures):}\edward{select the total tokens of caption are no more than 100 tokens}This collection only includes the figures whose caption's first sentence has no more than 100 tokens. For each figure included, this collection includes the maximum number of sentences (count from the beginning of the caption) \textbf{before exceeding 100 tokens}. \kenneth{THIS PART IS STRANGE. MAKE SURE YOU MAKE IT RIGHT.}

\item \textbf{Single-Sent Caption (94,110 figures):} This collection only includes the \textbf{figures with a one-sentence caption}. For each figure included, this collection includes the complete caption text. 

%\item \textbf{1st Sent (133,543 figures)\kenneth{CHECK NUMBER. This is incorrect!}:}\edward{this correct} This collection includes all the figures. For each figure included, this collection only includes \textbf{the first sentence} of the caption. 

\paragraph{Step 6: Target Caption Text Selection.}
Despite all the data processing and filtering strategies applied in the previous steps, the remaining figures still have quite diverse captions. To explore different data selection strategies, in \dataset, we provide three different data collections, each sampled using different strategies:


 \item \textbf{Advanced Normalization:} 
On top of the Basic normalization, we further perform a set of advanced normalization operations.
We first use ARQMat~\cite{mansouri2020finding}, which is powered by a rich set of regular expressions, to identify equations in captions and replace them with [EQUATION]. We then replace all the text spans enclosed by any types of bracket pairs, including \{\}, [], (), with [BRACKET]. 

\item \textbf{Basic Normalization:} 
    We use NLTK~\cite{Loper02nltk:the} first to tokenize all the words and convert all the characters to lower-case. We then replace all the numbers (numerical strings, {\em e.g.}, 0, 0.2, 3.44, 100) with [NUM]; we also remove the percentage sign (\%).

\paragraph{Step 5: Text Normalization.}
In \dataset, we apply the following two sets of text normalization strategies:


\paragraph{Step 4: Removing Figures with Multiple Subfigures.}
Many scientific figures contain more than one subfigures.
For example, in our pilot study (Section~\ref{sec:2000-figure-study}), 35.72\% of figures have subfigures.
\dataset focuses on generating captions for single figures, so we further remove figures with more than one subfigures from the dataset.
We first use a set of hand-crafted rules to identify the captions that explicitly mention or refer to the subfigures, for example, (a), a), (b), b), (1), 1), (2), 2) ... etc.
This rule-based approach yields a high classification precision (0.82 in graph plots) but a low recall (0.36 in graph plots). 
To increase the recall, we further use FigureSeparator~\cite{tsutsui2017data} to filter figures with multiple subfigures in our collection.
FigureSeparator is a CNN-based model that separates compound figures with an 85.9\% accuracy on the ImageCLEF Medical dataset.
As a result, out of 133,543 graph plots identified in the previous step\kenneth{CHECK NUMBER. This number is probably incorrect!}\edward{32.04\% are single figure, 67.96\% are multiple figures}, 32.04\% contain subfigures (283,261), which we remove from our dataset.

According to ths classifier's prediction, out of 2,170,719 figures, 19.2\% (416,804) are graph plots\kenneth{CHECK NUMBER}\edward{correct}, 23.6\% (511,984) are tables, 5.9\% (127,197) are equations (including algorithms and pseudo codes), 8.5\% (185,398) are flowcharts, 2.0\% (44,052) are scatter plots, 4.7\% (101,146) are bar charts, and 36.1\% (784,138) are other. 
In \dataset, we focus on \textbf{graph plots}, which has the highest classification performance~\cite{siegel2016figureseer} and are also the most common figure type.

In this work, we consider tables are not part of figure due to their drastically different visual features, contents, and usages. 


\paragraph{Step 3: Figure Type Classification.}
Given the extremely high diversity of figure types in scientific articles, we do not aim to create one single captioning model for all types of figures.
Instead, we aim to create captioning models specialized for one particular figure type.
We use an automatic figure type classifier~\cite{siegel2016figureseer} to classify figure type in \dataset.
This pre-trained classifier can identify seven types of figures: graph plots, flowcharts (also called node diagram), equations (also called algorithms), bar plots, scatter plots, tables, and other. 
Its reported accuracy is 86\% over 60,000 samples.


\paragraph{Step 2: Figure-Caption Pair Extraction.}

%because not all papers have source files

We then used PDFFigures 2.0~\cite{clark2016pdffigures} to extract the figures from papers from our paper collection.
PDFFigures 2.0 is a Scala-based tool created to extract figures, captions, tables, and section titles from scholarly documents with a strong focus on documents from the domain of computer science. 
%mention what information we also have
This step resulted in 295,028 papers and 2,170,719 figures.

In addition to the figures image and their captions, the tool also extracted the exact coordinates of above components and the text inside the figures. The extracted information can potentially be used to boost the performance image captioning models.

We first downloaded all the scholarly articles from the arXiv dataset and froze the date of data on Dec 22, 2020 (a total of 1,921,287 papers).
\dataset does not include any papers published after this date.
In particular, we selected the papers published between 2010 to 2020 in Computer Science (cs.) and Machine Learning (stat.ML) area,
%filtered by the meta-data information,
which included 295,028 papers. 
%in total. %should we mention why not use paper before 2010?
Note that we did not use the papers' source files, which might include the original latex files and figure files.
We did not use these source files because not all papers have source files.
Some paper's source files also have complex dependencies, which is not easy to parse.

Most prior works used synthesized data to train figure captioning models.
The real-world figures and captions, on the other hand, are much richer and also much nosier.
This section describes our process that massage the real-world figure caption data into a suitable, easy-to-use format for the NLP community.
This data processing procedure was developed iteratively and empirically.

To evaluate the quality of our data cleaning and processing pipeline, we randomly sample 2,000 figures (1926 valid figures without any recogniztion errors) from the original arXiv dataset and manually label the figure type and subfigures (Yes/No) of each image.
As for types, 20.35\% of figures are graph plot, 4.1\% of figures are bar charts, 3.11\% of figures are Scatter plots.
%add more type 
%mention the 2000 figure stats.

As for subfigures, 688 out of 1,926 contains subfigures, 33.14\% of subfigures are graph plot, 5.81\% of subfigures are bar charts, 6.83\% of subfigures are Scatter plots, 
%mention the 20000 subfigure stats.

We also evaluate the tools we use for figure classification. See the details in the following subsections.

\paragraph{Figure Type Classifier.}
The overall performance over graph plots and bar charts type are reliable, for graph plots in which the accuracy = 0.95, precision = 0.9, recall = 0.83 and F-1 = 0.87. for bar charts in which the accuracy = 0.99, precision = 0.85, recall = 0.78 and F1 = 0.81. 
%add numbers

\paragraph{Rule-Based Subfigure Classifier.}
This rule-based approach yields a high classification precision (0.82 in graph plots, 0.71 in bar charts), but a low recall (0.36 in graph plots, 0.17 in bar charts).

%mention the eval results

\paragraph{ML-Based Subfigure Classifier.}
The overall performance in graph plots are reliable as well, accuracy = 0.82, precision = 0.7, recall = 1.0 and F-1 = 0.82.

%mention the eval results

In the previous section, we mention the total valid figures of graph plots after removing the subfigures are 133,543. Although we rule out huge noisy images by above methods, the captions are still really diverse. Based on out data analysis, we found most of figures contain caption length (L) <= 11, especially when L = 1, they occupy 47.35\% among all captions. In here, we use three different targeted caption, (“1st Sent”, “Single-Sent Caption”, “First 100 Words”) , for training to see which category of captions perform well.

\begin{itemize}
    \item \textbf{1st Sent} All the images. Using only the first sentence in each caption. Total 133,543 valid figures. 
    \item \textbf{Single-Sent Caption} Only the images that the captions have only one sentence. Total 94,110 valid figures. 
    \item \textbf{First 100 Words} Only the images that the first sentence of the captions have no more than 100 tokens. Only use the sentences where the total \#token <= 100. Total 131,319 valid figures. 
\end{itemize}
%\paragraph{Data Analysis.}

Since the real caption data are pretty noisy, we first do several basic normalization to clean it before training and also check how it could impact the performance.
\begin{itemize}
    \item \textbf{Basic Normalization:} Basic (regular exp): Tokenization/Lower Case/Number/Percentage
    In here, we use NLTK~\cite{Loper02nltk:the} package to do lower case and tokenization on the captions that is very basic technique to clean the captions. We then replace the number with [NUM] token to avoid the real number. Then we also remove percentage “\%” which is usually following from digits. We name this step as "level 1 normalization"

    \item \textbf{Advanced Normalization:} Equation/Brackets (on top of a)
    We further do advanced normalization based on “level 1 normalization” to check if it could improve the performance. We use ARQMat~\cite{mansouri2020finding} that uses a lot of regex to identify math latex tags in the text and replace the equation with [EQUATION] in all figure caption data. Sometimes the bracket \{\}, [], (), represent additional notations that could noise the data, so we would like to avoid that as well. We replace the bracket with [BRACKET]. If it is a nested case in the caption, we will use the widest scope of bracket for replacement without considering the priority of bracket. We name this step as "level 2 normalization"
\end{itemize}

Many scientific figures would contain more than one subfigures.
For example, in our pilot study (Section~\ref{sec:2000-figure-study}), 35.72\% of figures have subfigures.
\dataset focuses on generating captions for single figures, so we further remove figures with more than one subfigures from the dataset.
We first use a set of hand-crafted rules to identify the captions that explicitly mention or refer to the subfigures, for example, (a), a), (b), b), (1), 1), (2), 2)... etc. This rule-based approach yields a high classification precision (0.82 in graph plots, 0.71 in bar charts), but a low recall (0.36 in graph plots, 0.17 in bar charts). To solve the problem, we further use Compound Figure Separator~\cite{tsutsui2017data}, a data driven method to separate compound figures using end-to-end pre-trained deep Convolutional Neural Networks (CNNs), which achieving 85.9\% accuracy on the ImageCLEF Medical dataset. Again, we evaluate the separator on the same 2,000 annotated figures that mentioned above. The overall performance in graph plots are reliable as well, accuracy = 0.82, precision = 0.7, recall = 1.0 and F-1 = 0.82.

% and outperforming manually engineered previous techniques. We made the resulting approach available as an easy-to-use Python library, aiming to promote further research in scientific figure mining.


% mention the tools and how it works.
% mention performance in the 2,000 set


As a results, out of 133,543 graph plots identified in the previous step, 32.04\% contain subfigures (283,261), which we remove from our dataset.
% mention the final number of figures included in the dataset


Given the extremely high diversity of figure types in scientific articles, we do not aim to create one single captioning model for all types of figures. Instead, we aim to create captioning models specialized for particular figure types. To this end, we use pre-trained classification model from ~\cite{siegel2016figureseer} to identify the figure types in our dataset. The classifier that can identify seven types of figures (Graph plots, Flowcharts(the authors renamed Node Diagram in their model later), Algorithms(the authors renamed Equation in their model later), Bar plots, Scatter plots, Tables and Other). In their paper, the classifier reach mean 86\% accuracy among 60,000 samples. The accuracy of each type is 89\%, 75\%, 77\%, 87\%, 59\%, 67\%, 93\% separately. We focus on Graph plots type that is the highest performance and it is also the most ratio (20.6\%) compared to other figure types not including other type, Flowcharts(12.6\%), Algorithms(6.8\%), Bar plots(6.1\%), Scatter plots(2.6\%), Tables(2.4\%). 

% Graph plots, Flowcharts, Algorithms, Bar plots, Scatter plots, Tables and Other). 

%report which types can it identify + mention its performance (reported in their paper)

As a results, out of 2,170,719 figures, 19.2\% (416,804) are graph plots, 23.6\% (511,984) are tables, 5.9\% (127,197) are equations, algorithms, pseudo codes(we renamed for more specific category), 8.5\% (185,398) are Node Diagram, 2.0\% (44,052) are Scatter plots, 4.7\% (101,146) are Bar charts, and 36.1\% (784,138) are Other. Although Tables type is the most among these figures (we do not consider other type), we still choose second amount, graph plots, as our target. Table type contains mostly text features that is really different from other's type. % not sure how to say ...


%mention figure types
We also manually annotate 2,000 figures (1,926 figures without errors) in our data collection to evaluate the classification model. We explain the details in Section~\ref{}.%say later

% The overall performance over graph plots and bar charts type are reliable, for graph plots in which the accuracy = 0.95, precision = 0.9, recall = 0.83 and F-1 = 0.87. for bar charts in which the accuracy = 0.99, precision = 0.85, recall = 0.78 and F-1 = 0.81. 
%add numbers

PDFFigures 2.0 built upon PDFFigures~\cite{clark2015looking} which has three main components, Caption Detection, Region Identification, and Figure Assignment. Caption Detection identifies words that mark the beginning of captions and uses Poppler library~\footnote{Poppler: https://poppler.freedesktop.org/.} contains Optical Character Recognition(OCR) technique to extract the text from the document. Region Identification aim to annotate the regions of each caption, graphical element, body text, or figure text in the whole document. Figure Assignment combine the figure and caption in pair. 
%describe the tools we used, and some technical details 
In addition to the figures image and their captions, the tool also extracted the exact coordinates of above components and the text inside the figures. The extracted information can potentially be used to boost the performance image captioning models.





Further, we extracted the figures from the selected PDF files, along with their caption texts. We used PDFFigures 2.0~\cite{clark2016pdffigures}, a Scala based project built to extract figures, captions, tables and section titles from scholarly documents, with a strong focus on documents from the domain of computer science, to extract the figures.

PDFFigures 2.0 built upon PDFFigures~\cite{clark2015looking} which has three main components, Caption Detection, Region Identification, and Figure Assignment. Caption Detection identifies words that mark the beginning of captions and uses Poppler library~\footnote{Poppler: https://poppler.freedesktop.org/.} contains Optical Character Recognition(OCR) technique to extract the text from the document. Region Identification aim to annotate the regions of each caption, graphical element, body text, or figure text in the whole document. Figure Assignment combine the figure and caption in pair. 
%describe the tools we used, and some technical details 
In addition to the figures image and their captions, the tool also extracted the exact coordinates of above components and the text inside the figures. The extracted information can potentially be used to boost the performance image captioning models.
%mention what information we also have


% 2. Explain which set of papers we used
We first downloaded all the scholarly articles from arXiv dataset and freezed the data before 12/22/2020 (total 1921287 papers). In particualr, since we target on scientific figures instead of general images, we select the papers published between 2010 to 2020 in Computer Science (cs.) and Machine Learning (stat.ML) fields filtered by the meta-data information, 295,028 valid papers in total. %should we mention why not use paper before 2010?

Note that we did not use the papers' source files, which might include the original latex files and figure files.
We did not use these source files because not all papers have source files.
Some paper's source files also have complex dependencies, which is not easy to parse.

%because not all papers have source files

we use PDFFigures 2.0~\cite{clark2016pdffigures}, a Scala based project built to extract figures, captions, tables and section titles from scholarly documents, with a strong focus on documents from the domain of computer science, to extract the figures from papers published between 2010 to 2020 in Computer Science (cs.) and Machine Learning (stat.ML) fields by the meta-data information on Kaggle arXiv daraset. There are 295,028 valid papers and 2,170,719 valid figures in total.


\end{comment}

%------------- dead kitten --------------

\begin{comment}


\paragraph{Step 1: Data Acquisition and Pre-processing.}
Data acquisition is a fundamental challenge for constructing a public scientific figures caption dataset.
Although there are a vast amount of scientific papers, they are not all easy to access.
% 1. Overview arXiv dataset
\dataset is constructed based on the arXiv dataset hold on Kaggle.\footnote{arXiv Dataset on Kaggle:\\ https://www.kaggle.com/Cornell-University/arxiv} %
arXiv dataset is licensed under CC-0, which allows remake and republish.
It contains a repository of 1.7 million articles, with relevant features such as article titles, authors, categories, abstracts, full text PDFs, and more. 
%In details, it composes of Metadata file and article in PDF format. 
%Metadata contains, id (ArXiv ID, can be used to access the paper), submitter (Who submitted the paper), authors (Authors of the paper), title (Title of the paper), comments (Additional info, such as number of pages and figures), journal-ref (Information about the journal the paper was published in), doi ([https://www.doi.org], Digital Object Identifier), abstract (The abstract of the paper), categories (Categories / tags in the ArXiv system), versions (A version history). PDF files are all hold on Google Cloud.
%explain what is in the arXiv dataset


\end{comment}

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/ethics.tex <==


%edited by MB
\paragraph{Data Licensing.}
The arXiv dataset uses the CC0 1.0 Universal (CC0 1.0) Public Domain Dedication license,\footnote{CC 1.0: \url{https://creativecommons.org/publicdomain/zero/1.0/}} which grants permission to remix, remake, annotate, and publish the data.



\paragraph{Potential Biases of Language Technologies.}
We are aware that language technologies	trained on a ``standard'' or mainstream variety of a language (in our case, English) favor the popular variety and harms people using varieties with fewer speakers.
For example, standard automatic speech recognition trained on Dutch speeches results in 10-15\% higher error rates on Flemish Dutch than on ``standard'' Dutch~\cite{feng2021quantifying}.

%---------------- dead kitten --------------

\begin{comment}


\paragraph{Potential Biases of Language Technologies.}
We are aware of that the language technologies trained on ``standard'' or mainstream variety of a language (in our case, English) would favoring the popular variety and harms the people using the varieties with fewer speakers.
For example, the standard automatic speech recognition trained on Dutch speeches results in a 10\% to 15\% higher word error rates on Flemish Dutch than that of on ``standard'' Dutch~\cite{feng2021quantifying}.

\paragraph{Data Licensing.}
The arXiv dataset uses CC0 1.0 Universal (CC0 1.0) Public Domain Dedication license,~\footnote{CC 1.0: https://creativecommons.org/publicdomain/zero/1.0/} which permits use to remix, remake, annotate, and publish the data.

\end{comment}

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/experiments.tex <==
%\input{table-new.tex}

% \input{train_val_test_size}

\input{new-table-with-data-size}

\input{v-and-t-table.tex}





%edited by MB
To examine the feasibility and challenges of creating an image-captioning model for scientific figures, we established several baselines and tested them using \dataset.
The caption quality was %automatically 
measured by BLEU-4~\cite{papineni2002bleu}, using the test set of the corresponding data collection as a reference.
Figure~\ref{fig:example} shows some example outputs.


%edited by MB
\paragraph{Baseline Model.}
\cy{I also rewrite the model description. Please check. @Edward please check if there is anything wrong.}
We used a classical image-captioning model, CNN+LSTM architecture, as our baseline~\cite{xu2015show}.
The pre-trained ResNet-101~\cite{he2016deep} was used as the image encoder to represent a figure as a 2048-dimension vector.
This image vector was then fed into a dense layer to fit the dimension of the word-embedding and the LSTM decoder where 
the word-embedding and LSTM hidden layer size were all 512.
A global attention mechanism was added to the LSTM decoder to better model the context~\cite{luong2015effective}.
The LSTM decoder took the image vector as the initial state and generate captions.

We designed three variations of the baseline models, Vision-only, Vision+Text, and Text-only.
The text information was the titles, legends, and X-Y labels extracted from the figures (Step 2 in Section~\ref{sec:dataset-construct}).
Another LSTM was used as a text encoder to encode text information into a vector.
For the Vision+Text variation, we concatenated the image vector and the text vector together 
and fed it into the LSTM decoder for caption generation.
The Text-only variation only took the text vector as the feature for the LSTM decoder.




\begin{figure*}[t]
\centering
\includegraphics[width=0.91\textwidth]{figures/example-figure.png}
%\vspace{-.5pc}
\caption{Example outputs of the baseline models trained and tested on the Single-Sentence Caption Only collection.
Intensive research will be needed to create models that can caption scientific figures reliably. 
[Figure sources: (1)~\cite{zhang2020protograph}, (2)~\cite{baswana2017incremental}, and (3)~\cite{brubaker2015building}.]}
\label{fig:example}
%\vspace{-.7pc}
\end{figure*}

%edited MB
\paragraph{Experimental Setups.}
We trained the baseline models using an 80/10/10 train/val/test data split.
The models were trained by minimizing a cross-entropy loss with a doubly stochastic regularization~\cite{xu2015show}
using Adam~\cite{kingma2014adam}.
The weights of the pretrained ResNet-101 image encoder were partially frozen so that only 
convolutional blocks 2 through 4 were fine-tuned throughout the training process~\cite{yosinski2014transferable}.
We empirically set the hyper-parameters by observing the performance gain on the validation set.
Hyper-parameters ended up being used were a dropout rate of 0.5; a batch size of 16/32; 
a learning rate of 4e-4 with a decay factor of 0.8 when there was no improvement for 8 epochs.
The models were trained until there was no improvement for 20 epochs.
We kept the model with the highest BLEU-4 score on the validation set for testing.


%We implement the following models with Pytorch, and conduct experiments on a single nVidia GeForce RTX 2080 GPU. 

%}\edward{do we need to give our model details?}

\paragraph{Results.}
%\kenneth{!!!This part needs to rewrite to fit in the new table.}
%Note that 
We trained the %baseline 
models on each data collection with varying levels of data filtering and text normalization.
Table~\ref{tab:text-only-result} shows the results.
%As mentioned in the Step 3 of Section~\ref{sec:dataset-construct}, FigureSeperator %different combined settings of data.
%As defined previously, 
%Text Data represented different targeted captions; 
%Cleaning Method represented different subfigure classification; 
%Text Normalization represented post-processing captions;
%Feature represented the information we used as training data; 
%and the last column displays the performance of generated captions.
%edited by MB
%\paragraph{Evaluations.}
%We report baseline models' performances in Table~\ref{tab:text-only-result}.
Among the three data collections, the models trained on the single-sentence captions performed the best. %\kenneth{This need to update later...}
This might be because the Single-Sentence Caption collection, which is a subset of the First Sentence collection, 
had the smallest vocabulary size.
%This might be because the first sentence of a caption is often the topic sentence, and thus has a lower lexical diversity.
%\cy{Is this true? Do we have numbers? As ``Single-sentence'' is a subset of ``First-sentence'', I feel it might have a even lower lexical diversity? I am not really sure about the relationship between ``topic sentence'', ``lower lexical diversity'', and ``performance''.}
%\kenneth{You're right, MAYBE it's just data size is lareger?}


%edited by MB
\paragraph{Effects of Text Normalization.}
%We performed different degrees of text normalization in \dataset to see whether text normalization could increase the quality of the generated captions. 
Our experiments did not show the clear benefits of normalizing text to the resulting BLEU-4 scores.
We will explore other methods to normalize text, for example, using advanced techniques to identify equations in text~\cite{mali2020scanssd,mansouri2020finding}.

%We adapted the regular expressions used in ARQMat~\cite{mansouri2020finding}, which was created to recognize equations in LaTeX codes, 
%which is powered by a rich set of regular expressions, 

%edited by MB
\paragraph{Effects of Text and Vision Features.}
%\kenneth{Add some text to describe new tables}
We also used Vision-Only, Text-Only, and Text+Vision features to develop models (Table~\ref{tab:text-and-vision-result}). 
%Our experiments showed that 
Vision-Only and Text-Only features yielded similar performance.
%The models performed similarly when using either Vision-Only or Text-Only features.
Furthermore, the models performed slightly worse when training on combined features.
%One possible reason is that the quality of the text extracted from the figures was low, thus introducing more noise than useful information into the model.
%\kenneth{We removed the data settings of V+T experiments from the Table. Can we describe the setups in text? Subfig figuring setting and normalization setting}







%\paragraph{Error Analysis.}
%Although we obtain the best performance from subfigures classification and text normalization technique, the BLEU-4 score is still pretty low in general. We check the generated captions from different setting. It is also hard to tell which one is better due to the low difference of BLEU-4 scores. 


%------------ dead kitten -------------

\begin{comment}


\kenneth{This part also needs some work}
%\kenneth{The texts are rough in this section. Need some more work.}
We used a CNN + LSTM architecture as our baseline.
This architecture is a typical baseline framework used for image-captioning tasks~\cite{xu2015show}.
%\kenneth{1. Image encoder here:}
We extracted the image features using the pre-trained ResNet-101 model~\cite{he2016deep} and represented each figure as a 2048-dimension vector.
We then fed the vector into a dense layer to fit the word-embedding dimension. %and learn the adjusting transformation.
%\kenneth{Q for Ed: This sentence is somewhat weird. What exactly did you mean?}\edward{this is what typical image captioning (CNN+RNN) model do, I don't understand your problem.}
%\kenneth{Is ``learn the adjusting transformation'' a standard way to describe this process? It reads somewhat strange.} \edward{we can remove learn the adjusting transformation}
%edited
%\paragraph{Text Feature (Used in Table~\ref{tab:text-and-vision-result}).}
%\kenneth{2. Add a sentence about how to use text feature here:}
In addition to image features, we also used the texts extracted from the figures (Step 2 in Section~\ref{sec:dataset-construct}) as features.
%\kenneth{MAYBE Say slightly more about the experiments: why doing this? what's the setup?}
%Table~\ref{tab:text-and-vision-result}) shows the results.
%\kenneth{So did you just concat the vectors?}\edward{yes}
%\edward{we would like to know whether use the key words information (image text) could construct reasonable sentences}
%\cy{Only the image-encoder is described here. How about the caption generation part (LSTM). How do you use the text as the features? What are these texts? Are they ``title'', ``legends'', and ``labels''? If so, it should probably be Step 2?}
%\kenneth{TODO: Explain LSTM/generator model here:}
In the decoder part, we used LSTM network to generate a caption word by word at each time step based on the previous hidden state and generated words. 
For the ``Text Only'' setting, we treated image text extracted the figure only and descriptive caption as pairs, using seq2seq LSTM model which is similar to Machine Translation technique\kenneth{not finished yet}




%where the text extracted were extracted from (inside) the figures.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Experimental Setups.}
%\kenneth{NEED MORE WORk HERE!!!}
%\edward{

%For each of them, we used pretrained ResNet-101\cite{} as the encoder, word embdding dimension = 256/512, attention linear layers dimension = 256/512, decoder dimension = 256/512. 

%\kenneth{I rearranged some texts in the paragraph. Please check if they're correct}
%\kenneth{The texts are rough in this section. Need some more work.}
\kenneth{TODO: CY can you rewrite this part to make it more clear.}
The baseline models were developed using
%For the experiments, we used 
an 80/10/10 train/val/test data split.
We used a pre-trained ResNet-101~\cite{he2016deep} as the encoder.\footnote{emb\_dim = 256/512, attention\_dim = 256/512, decoder\_dim = 256/512} %which is optimized by Adam~\cite{}
The model was trained by a cross-entropy loss with a doubly stochastic regularization~\cite{xu2015show}
%with doubly stochastic regularization.
%After max pooling, a dropout layer is added with a 
(dropout rate = 0.5.)
We tried different parameter combinations and kept the best setting. \cy{Any information on the parameter searching? What were the hyperparameters you tried? What were their range?}\edward{greedy search of different dimension settings and batch size}
The optimization was performed using
%All of them are optimized with 
Adam~\cite{kingma2014adam}; 
%on the training set and evaluated on the testing set. 
%We tune 
the hyperparameters were tuned on the validation set.

We used a batch size of 16/32. 
\cy{What the slash mean?}\edward{try different batch size} %due to the limitation of GPU resources.
The learning rate was decayed by a factor of 0.8 if there was no improvement occurred for 8 consecutive epochs.
%do early stopping with BLEU-4 after 20 epochs; emb\_dim = 256/512, attention\_dim = 256/512, decoder\_dim = 256/512. 
We also applied early stopping %to prevent overfitting
%. More specifically, we stopped the training procedure 
when the BLEU-4 score on the validation set did not improve for 20 consecutive epochs.
%reaches the maximum.
The encoder was also fine-tuned. \cy{What does this mean? The encoder is fine-tuned separately or what?}\edward{We also want to fine-tune the Encoder, we add a fine tune function which enables or disables the calculation of gradients for the Encoder's parameters. We only fine-tune convolutional blocks 2 through 4 in the ResNet, because the first convolutional block would have usually learned something very fundamental to image processing, such as detecting lines, edges, curves, etc.}
%We used CrossEntropyLoss and a second loss (``doubly stochastic regularization'') as suggested in [1]. \edward{we use dropout=0.5}
%We trained 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Effects of Text Normalization.}
We perform different degrees of text normalization in \dataset to see whether text normalization could help with generated caption quality.
Our experiments show that text normalization did help improve the performance, measured by BLEU-4, in all settings. The improvements are, admittedly, minor, but we believe text normalization is a promising direction to explore.


\paragraph{Effects of Text and Vision Features.}
We use vision-only, text-only, and text+vision features, respectively, to observe their effects.
Our experiments show that models can learn better from vision-only features compared with text-only features. Furthermore, models perform even worse when training on the combined features. 
A possible reason is that the quality of the text extracted from the figures is low and thus introduces more noise than useful information to the model.

\paragraph{Evaluations.}
We report baselines' performance on \dataset in Table~\ref{tab:baseline-results}. 
Among three data collections (Step 6 in \S\ref{sec:dataset-construct}), the models trained on the first sentence of figure captions perform the best.
This might be caused by the fact that the first sentence of a caption is often the ``topic sentence'' and thus have a lower lexical diversity.

\paragraph{Experiment Setups.}
We trained the baseline models on different combined setting of data.
Each column's property has been already introduced in the previous sections. Text Data represented different targeted caption, Cleaning Method represented the different subfigures classification, Text Normalization represented the post-processing captions, Feature represented what information we used as training data, and the last column is the performance of generated captions. 
%\kenneth{You should explain what is the TEXT feature. It's unclear.}

\paragraph{Text Feature (T in Table 1).}
In addition to im-	272
age features, we also used the texts extracted from	273
the figures (Step 3 in §3) as text features.

\paragraph{Baseline Model.}
We use a CNN + LSTM architecture as our baseline. 
This architecture is a typical framework used for image captioning tasks~\cite{xu2015show}. 
We extract the image features using the pre-trained ResNet-101 model~\cite{he2016deep} and represent each figure as a 2048-dimension vector.
We then feed the vector into a dense layer to fit the dimension of word embedding and learn the adjusting transformation.


To examine the feasibility and challenges of creating a usable image captioning model for scientific figures, we establish a set of baselines and test them on \dataset.


\end{comment}

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/intro.tex <==
% Kenneth: I did a sentence-by-sentence re-write based on your text. Try to use simple, direct, short sentences in your future writing.

%\lee{Hi Lee, you can use \lee{} to add comments! }

%\kenneth{(1) We will need to pick one or two examples from the data set. I want a few examples of Graph Plot (image) and show their captions (text) that go through Step 1, 2, ..., 6. Showing how we processed/normalized the data.}




Researchers use figures to explain complex concepts or show critical results.
In scholarly articles, figure captions are critical to get the message across effectively.
Ones that are too generic ({\em e.g.}, ``Results of Experiment A.'') or poorly written ({\em e.g.}, ``Relations between X and Y.'') represent missed opportunities to explain scientific narratives to readers.
Unfortunately, such low-quality captions still occur in published scientific articles.
%To address this, we will develop automated figure captioning models that generate high-quality captions for figures and charts in scientific papers (Figure~\ref{fig:overview}). Our aim is two-fold.
This paper aims to develop automatic figure-captioning models that generate high-quality captions for figures and charts in scientific papers (Figure~\ref{fig:overview}).
%Our aim is two-fold.
%Such models take a scientific figure ({\em e.g.}, a graph plot) as input and generate a caption that describes the figure.


\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/overview-larger-font.png}
%\vspace{-1.5pc}
\caption{The figure captioning model takes a scientific figure ({\em e.g.}, a graph plot) as input and generate captions that describes the figure.}
\label{fig:overview}
%\vspace{-1pc}
\end{figure}


%edited by MB
Our motivation is two-fold.
First, we aim to help researchers write better captions for the figures and charts in their papers.
Automatic caption models trained on informative, high-quality captions can suggest better captions.
Second, the proposed technology can make scientific charts and figures more accessible to blind or visually impaired readers.
Researchers have developed technologies to assist the blind to navigate graphical content, such as data visualization charts~\cite{swaminathan2014supporting}, 
printed physical maps~\cite{swaminathan2016linespace}, 
3D chemical diagrams~\cite{bernareggi2019mugraph}, 
and images on social media~\cite{wu2017automatic,salisbury2017toward}.
However, only a few prior works focused on scientific figures.
An image-captioning model specialized for scientific figures can improve the narration of scientific articles for the blind even when the original caption is unhelpful.




%edited
To this end, we introduce \textbf{\dataset}, a large-scale image-captioning dataset that contains real-world scientific figures and captions.
\dataset was constructed using computer science papers collected and released by arXiv.
With pre-processing complete -- including figure-type classification, sub-figure identification, text normalization, and caption text selection -- 
\dataset contained more than two million figures extracted from over 290,000 papers.
%\kenneth{We might want to be more specific here. What exactly are we going to release?}\edward{Didn't we plan to release the single graphplot figure? (all figures and preprocessed data)}\kenneth{But we didn't plan to release all 2M figures. We will not release the unprocessed or removed ones.}\edward{what I mean is release single graphplot figure and captions}
We then established baseline models that caption graph plots, the dominant (19.2\%) figure type.
The experimental results 
%We also established several image-captioning baselines, 
showed both exciting opportunities and steep challenges of generating captions for scientific figures.


%We developed image-captioning models for graph plots, the dominant (19.2\%) figure type.
%Experiments show that the proposed framework produces better captions than other baselines\kenneth{AGAIN THIS IS NOT TRUE}, shedding light on the possibilities of future automatic writing support options for figure captions.







%--------------------- dead kitten ------------

\begin{comment}


%edited by MB
%Researchers use figures to communicate rich and complex information in scientific papers.
%The captions of these figures are critical to convey the messages effectively.
%However, low-quality figure captions that do not enhance comprehension, such as ``Results of Experiment 1,'' occur commonly in scientific articles.
%This paper aims to develop automatic image captioning models that generate high-quality captions for figures and charts in scientific papers.
%Such models take a scientific figure ({\em e.g.}, a graph plot) as input and generate a caption that describes the figure.

% \kenneth{UPDATE NUMBERS ACCORDINGLY}
To this end, we introduce \textbf{\dataset}, a large-scale image captioning data that contains real-world scientific figures and captions.
\dataset was constructed using the papers collected and released by arXiv.
After pre-processing --- including figure type classification, sub-figure identification, text normalization, and caption text selection --- \dataset contains more than two million figures were extracted from over 290,000 papers.
% We focus on graph plots which is the most dominant and clear defined category of scientific figures. We further develop neural image caption models that generate high-quality captions for those figures.
We then develop image captioning models for graph plots, which is the dominant (19.2\%) figure type.
% Experiments show that our proposed framework can generate reasonable captions for scientific figures under several metrics and outperforms the baselines in human aspects, thus claiming a significant potential for the automatic detailed captioning of scientific figures.
Experiments show that the proposed framework produce better captions than other baselines, shedding lights on the possibilities of future automatic writing supports for figure captions.



Our motivation is two-fold.
First, we aim to help researchers write \textit{better} captions for the figures and charts in their papers.
%``Placeholder captions'' --- such as ``Results of Experiment 1'' --- do not help readers understand but occur commonly in academic articles.
When researchers write papers, automatic caption models trained on informative, high-quality captions can suggest better captions.
Second, the proposed technology can further make scientific charts and figures more accessible to blind or visually impaired readers.
Researchers have been developing technologies to assist the blind navigate graphical content, such as data visualization charts~\cite{swaminathan2014supporting}, printed physical maps~\cite{swaminathan2016linespace}, 3D chemical diagrams~\cite{bernareggi2019mugraph}, and images on social media~\cite{wu2017automatic,salisbury2017toward}.
However, only a few prior works focused on scientific figures.
An image captioning model specialized for scientific figures can narrate scientific articles for the blind better even when the original caption is unhelpful.

% Figures contain rich and useful information that is human friendly to read due to the inherency of visual format. In certain formats, such as graph plots, bar charts, tables, especially in scientific fields have been widely using to help people better understand the data representation. 
Researchers use figures to communicate rich and complex information in scientific papers.
%
% People also use machines to process those data efficiently. --> I removed this one. It's not relevant to your core argument.
%
% Although figures are straightforward for humans to read, sometimes it could be confused for non-domain experts or people who are working outside this specific field to realize the core concept of the figures. And further, lots of descriptive captions of those figures are ambiguous and do not provide any detailed information. 
The captions of these figures are critical to convey the messages effectively.
%
% Not to mention that it is even harder for machines to process them. --> Removed again. "Help computer" is NOT your core motivation.
%
% In the paper, we propose a novel end-to-end framework to automatically generate captions for scientific figures. --> Don't jump to "what you do". You will need a "HOWEVER" first.
However, low-quality figure captions, such as ``Results of Experiment 1'',
occur commonly in scientific articles, which do not help, or even hurt, understanding. %This is the HOWEVER.
This paper aims to develop neural image caption models that generate high-quality captions for figures and charts in scientific papers.
Such models take a scientific figure ({\em e.g.}, a graph plot) as input and generate a caption that describes the figure.

This paper aims to develop neural image caption models that generate high-quality captions for figures and charts in scientific papers.
Such models take the image of a scientific figure ({\em e.g.}, a graph plot) as input and generate text captions that describe the figure to generate a new and better caption.
The motivation is two-fold.
First, we aim to help researchers to write better captions for the figures and charts in their papers.
``Placeholder'' captions, such as ``Evaluation Results of Experiment 1'', do not help understanding, yet occur commonly in academic articles.
When researchers write papers, neural caption models trained on informative high-quality captions can be used to suggest better captions.

Second, the proposed technology can further make scientific charts and figures more accessible to blind or visually impaired audience.
Researchers have been developing technologies to assist the blind navigate graphical content, such as data visualization charts~\cite{swaminathan2014supporting}, printed physical maps~\cite{swaminathan2016linespace}, 3D chemical diagrams~\cite{bernareggi2019mugraph}, and images on social media~\cite{wu2017automatic,salisbury2017toward}.
However, none of the prior work focused on scientific figures at large.
Equipped with an automated image captioning model, these models will be able to better narrate scientific figures and charts to the blind even when the original caption is not very helpful.



\end{comment}


==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/new-table-with-data-size.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multicolumn{7}{c}{\cellcolor[HTML]{EFEFEF}\textbf{First Sentence}} \\ \midrule
\multicolumn{2}{c}{\textbf{Subfig Filter}} &
  \multicolumn{2}{c}{\textbf{Norm.}} &
   &
   &
   \\ \cmidrule(r){1-4}
\textbf{Rule} &
  \textbf{FigSep} &
  \textbf{B.} &
  \textbf{A.} &
  \multirow{-2}{*}{\textbf{\#Fig.}} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Vocab\\ Size\end{tabular}}} &
  \multirow{-2}{*}{\textbf{BLEU-4}} \\ \midrule
 &
   &
   &
   &
  416,804 &
  30,776 &
  .0259 \\ \midrule
\cmark &
   &
  \cmark &
   &
  352,719 &
  24,355 &
  .0236 \\ \midrule
\cmark &
  \cmark &
  \cmark &
   &
   &
  12,666 &
  .0224 \\ \cmidrule(r){1-4} \cmidrule(l){6-7} 
\cmark &
  \cmark &
  \cmark &
  \cmark &
  \multirow{-2}{*}{133,543} &
  11,946 &
  .0219 \\ \midrule
\multicolumn{7}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Single-Sentence Caption Only}} \\ \midrule
\multicolumn{2}{c}{\textbf{Subfig Filter}} &
  \multicolumn{2}{c}{\textbf{Norm.}} &
   &
   &
   \\ \cmidrule(r){1-4}
\textbf{Rule} &
  \textbf{FigSep} &
  \textbf{B.} &
  \textbf{A.} &
  \multirow{-2}{*}{\textbf{\#Fig.}} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Vocab\\ Size\end{tabular}}} &
  \multirow{-2}{*}{\textbf{BLEU-4}} \\ \midrule
 &
   &
   &
   &
  247,649 &
  21,765 &
  .0291 \\ \midrule
\cmark &
   &
  \cmark &
   &
  218,655 &
  17,685 &
  .0228 \\ \midrule
\cmark &
  \cmark &
  \cmark &
   &
   &
  9,760 &
  .0234 \\ \cmidrule(r){1-4} \cmidrule(l){6-7} 
\cmark &
  \cmark &
  \cmark &
  \cmark &
  \multirow{-2}{*}{92,021} &
  9,232 &
  .0207 \\ \midrule
\multicolumn{7}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Caption with \textless{}= 100 Words}} \\ \midrule
\multicolumn{2}{c}{\textbf{Subfig Filter}} &
  \multicolumn{2}{c}{\textbf{Norm.}} &
   &
   &
   \\ \cmidrule(r){1-4}
\textbf{Rule} &
  \textbf{FigSep} &
  \textbf{B.} &
  \textbf{A.} &
  \multirow{-2}{*}{\textbf{\#Fig.}} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Vocab\\ Size\end{tabular}}} &
  \multirow{-2}{*}{\textbf{BLEU-4}} \\ \midrule
 &
   &
   &
   &
  395,024 &
  37,885 &
  .0231 \\ \midrule
\cmark &
   &
  \cmark &
   &
  341,350 &
  30,316 &
  .0098 \\ \midrule
\cmark &
  \cmark &
  \cmark &
   &
   &
  15,642 &
  .0173 \\ \cmidrule(r){1-4} \cmidrule(l){6-7} 
\cmark &
  \cmark &
  \cmark &
  \cmark &
  \multirow{-2}{*}{132,120} &
  14,974 &
  .0172 \\ \bottomrule
\end{tabular}
%\vspace{-.5pc}
\caption{The baseline model's performance on \dataset, using Vision-Only features.
Models trained on the Single-Sentence Caption collection performed the best.
%; normalizing caption improves the model's performance.
%; the text information (T) extracted from figures does not help the models. 
The low BLEU-4 scores indicate that more research is needed to reliably generate captions for scientific figures. 
%\kenneth{The vocab size is BEFORE pruning, right?}
(The vocabulary sizes were calculated after dropping words with a frequency below 5.)
%\kenneth{TODO: Move all the numbers to the new table}
}
%\vspace{-1.2pc}
\label{tab:text-only-result}
\end{table}

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/old_emnlp_instruction.tex <==

These instructions are for authors submitting papers to EMNLP 2021 using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} as well as guidelines set forth in the EMNLP 2021 call for papers. This document contains additional instructions for the \LaTeX{} style files.

The templates include the \LaTeX{} source of this document (\texttt{emnlp2021.tex}),
the \LaTeX{} style file used to format it (\texttt{emnlp2021.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{emnlp2021}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{emnlp2021}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
\citealp{Gusfield:97} & \verb|\citealp| & no equivalent \\
\citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

% \nocite{Ando2005,borschinger-johnson-2011-particle,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{custom}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.



\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.


==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/related_work.tex <==
%The work is related to 
%{\em (i)} applications of automatic image captioning and
%{\em (ii)} technical supports for visual storytelling.

%and
%{\em (iii)} storytelling using images.

\begin{comment}


\paragraph{Applications of Image Captioning.}
Image captioning has been used to generate alternative text for images on the Internet, helping blind users navigate web pages.
Macleod {\em et al.} studied the blind's reaction to machine-generated image captions in the context of navigating online social media platforms~\cite{macleod2017understanding}.
They found that the blind tend to over-trust AI systems, even when the generated captions do not make sense.
They suggested that automatic intelligent systems should better communicate their uncertainty to users.
Researchers have developed systems to improve and polish machine-generated captions to help the blind, for example, using real-time crowdsourcing~\cite{salisbury2017toward} or reverse image search~\cite{guinness2018caption}.
Another common application is to support personal sharing.
For example, AutoCaption is a mobile application that performs a set of computer vision tasks, including face recognition,
landmark recognition, and scene recognition on photos. It then creates personalized image captions that can be shared on the social media~\cite{ramnath2014autocaption}.
Zhao {\em et al.} also developed a system that automatically captions photos for the blind before they share pictures to Facebook~\cite{zhao2017effect}.


\end{comment}


%edited MB
One of the few prior works attempting to caption scientific figures was by Chen {\em et al.}~\shortcite{Chen:2019:NCG:3341162.3345601,chen2019figure,chen2020figure}.
%\edward{\cite{chen2019figure}\cite{chen2020figure}}.
%Chen {\em et al. to caption scientific figures~\shortcite{Chen:2019:NCG:3341162.3345601}.
They created FigCAP, a caption-figure pair corpus where the figures are synthesized, and used an LSTM model with an attention mechanism to produce captions.
%This work is inspiring and relevant, but it did not	use real-world figure-caption pairs. 
%\kenneth{Move text from rebuttal or Adobe Proposal to explain WHY}
%Chen explained that they used synthetic data because the realistic dataset was relatively small.
%In this paper, we take advantage of the large-scale paper dataset collected and release by arXiv to develop our model.
%Furthermore, 
FigCAP was built on research that aimed to analyze figure content automatically,
%in figure understanding, which attempted to analyze figure content automatically.
%is the extraction of the plotted data and its association
%with the legend entries
%This 
including Figure-Seer~\cite{siegel2016figureseer}, 
FigureQA~\cite{kahou2017figureqa}, and
DVQA~\cite{kafle2018dvqa}.
%The figures in both 
DVQA and FigureQA were both made using synthetic figures;
FigureSeer contained over 60,000 figures across seven figure types extracted from research papers.
Meanwhile, Qian {\em et al.}~\shortcite{qian2020formative} proposed a set of ``caption units'' (such as Title, Label Name, Min/Max, etc.) that are important to include in a caption of scientific figures; they created a model, FigJAM, to produce such units~\cite{qian2021generating}.
%Chart-to-Text: Generating Natural Language Descriptions for Charts by Adapting the Transformer Model
%An overview of the proposed approach for chart summarization using a transformer-based model. 
%The model takes the data table and some chart metadata as input (on the left) and generates a summary containing data
%variables that refer values within the data table
%Neural Data-Driven Captioning of Time-Series Line Charts
Also relevant is the ``data-to-caption'' work, which takes a chart's source data table and metadata as input to generate a caption~\cite{obeid2020chart,spreafico2020neural}.
These models generate captions based on data tables, not the figures.
%well-known “six hats” method, which asks
%people to wear metaphorical hats representing different thinking perspectives [10]. Teevan et al. proposed to use the six
%hats schema to assign different thinking roles to the authors
%themselves in order to promote self-reflection from different
%angles [38]. Chou et al. showed that perspective-taking can


%that achieves this goal through utilizing metadata
%information and a joint static and dynamic dictionary



%Our study results show that real-world captions usually consist of a finite set of caption units and that automatic figure
%captioning should be formulated as a multi-stage task.

%\kenneth{WHY it's different?}
%\kenneth{Add Xin's CHI LBW and WWW papers.} \cite{qian2021generating}\cite{qian2020formative}\edward{added}


\paragraph{Differences Between Synthetic and Real-World Captions.}
%Using human-written captions to develop captioning models will allow us to understand how scientists write captions in papers.
Most prior work has tried to generate captions for scientific figures using synthetic images and texts~\cite{Chen:2019:NCG:3341162.3345601,chen2019figure,chen2020figure,kahou2017figureqa}.
%\edward{\cite{chen2019figure}\cite{chen2020figure}}
%Real-world captions are better because they encode the realistic languages used in scientific captions.
However, synthetic captions tend to be generic and describe features without conveying higher-level insights,
for example,
\textit{``This is a line plot. It contains 6 categories. Dark Magenta has the lowest value. Lawn Green has the highest value.''} (example from FigCAP.)
%\edward{\cite{chen2019figure}\cite{chen2020figure}}.\kenneth{Is this example indeed from this dataset? What's the dataset name?}\edward{real example from FigCAP}
Human-written captions, on the other hand, tend to highlight the meaningful parts of the figure and bring more context, for example: 
\textit{``Train loss curve with respect to optimization steps. With prior coarse-tuning on NLI data, convergence becomes much faster and easier.''}
%Example of learning curve for unigram BLEU score. Red line is the exact BLEU score obtained by... Purple dotted line is... Crosses denote expected BLEU score calculated by averaging samples from distri- bution px.
[example from~\cite{jin2020mmm}].
%Synthetic captions cover all the visual detail of a figure equally, for example,
%\textit{``This is a line plot. It contains 6 categories. Dark Magenta has the lowest value. Lawn Green has the highest value.''} (example from~\cite{Chen:2019:NCG:3341162.3345601}).



%------------------ dead kitten ---------------------

\begin{comment}

%\paragraph{Scientific Figure Understanding and Captioning.}
One of the few prior works attempted to caption scientific figures was done by Chen {\em et al.}~\cite{Chen:2019:NCG:3341162.3345601}\cite{chen2019figure}\cite{chen2020figure}.
They created FigCAP, a caption-figure pair dataset where the figures are synthesized, and used an LSTM model with attention to produce captions.
This work is inspiring and relevant, but it did not use real-world figure-caption pairs.
Chen explained that they used synthetic data because the size of the realistic dataset is relatively small.
In this paper, we take advantage of the large-scale paper dataset collected and release by arXiv to develop our model.

Furthermore, FigCAP was builds upon the research in figure understanding, including FigureSeer~\cite{siegel2016figureseer}, FigureQA~\cite{kahou2017figureqa}, and DVQA~\cite{kafle2018dvqa}. FigureSeer contains real figures from research papers, but the figures in both DVQA and FigureQA are synthetic.


Figures are human-friendly but difficult for computers to process automatically. In this work, we investigate the problem of figure captioning. The goal is to automatically generate a natural language description of a given figure. We create a new dataset for figure captioning, FigCAP. To achieve accurate generation of labels in figures, we propose the Label Maps Attention Model. Extensive experiments show that our method outperforms the baselines. A successful solution to this task allows figure content to be accessible to those with visual impairment by providing input to a text-to-speech system; and enables automatic parsing of vast repositories of documents where figures are pervasive.

%FigureQA contains bar charts, pie charts, line plots, and dot-line plots while DVQA has only bar charts.
In~\cite{Chen:2019:NCG:3341162.3345601},

In this sense, the size of
FigureSeer is relatively small compared to DVQA and FigureQA,
though its figures come from real data. 




on top of figure \textit{understanding}

a synthetic dataset where 


There are some public datasets from previous work
on figure understanding, such as FigureSeer [13], DVQA[5] and
FigureQA [6]. FigureSeer contains figures from research papers,
while plots in both DVQA and FigureQA are synthetic. Due to the
synthetic nature, one can generate as many figures, accompanied
by questions and answers as he wants. In this sense, the size of
FigureSeer is relatively small compared to DVQA and FigureQA,
though its figures come from real data. In terms of figure type,
FigureQA contains vertical and horizontal bar charts, pie charts,
line plots, and dot-line plots while DVQA has only bar charts. Also,
reasoning ability is important for captioning approaches to generate
good quality captions. Note that FigureQA is designed for visual
reasoning task. Considering the above factors, we generate our
dataset FigCAP based on FigureQA.


\end{comment}

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/table-new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{@{}cccccc@{}}
\toprule
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{First Sentence} (133,543 graph plots)} \\ \midrule
\multicolumn{2}{c}{\textbf{Subfig Filtering}} &
  \multicolumn{2}{c}{\textbf{Normalization}} &
   &
   \\ \cmidrule(r){1-4}
\textbf{Rule} &
  \textbf{FigSep} &
  \textbf{Basic} &
  \textbf{Adv} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Vocab\\ Size\end{tabular}}} &
  \multirow{-2}{*}{\textbf{BLEU-4}} \\ \midrule
   &
   &
   &
   &
  30,776 &
  .0259 \\ \midrule
\cmark &
   &
  \cmark &
   &
  24,355 &
  .0236 \\ \midrule
\cmark &
  \cmark &
  \cmark &
   &
  12,666 &
  .0224 \\ \midrule
\cmark &
  \cmark &
  \cmark &
  \cmark &
  11,946 &
  .0219 \\ \midrule
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Single-Sentence Caption} (94,110 graph plots)} \\ \midrule
\multicolumn{2}{c}{\textbf{Subfig Filtering}} &
  \multicolumn{2}{c}{\textbf{Normalization}} &
   &
   \\ \cmidrule(r){1-4}
\textbf{Rule} &
  \textbf{FigSep} &
  \textbf{Basic} &
  \textbf{Adv} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Vocab\\ Size\end{tabular}}} &
  \multirow{-2}{*}{\textbf{BLEU-4}} \\ \midrule
 &
   &
   &
   &
  21,765 &
  .0291 \\ \midrule
\cmark &
   &
  \cmark &
   &
  17,685 &
  .0228 \\ \midrule
\cmark &
  \cmark &
  \cmark &
   &
  9,760 &
  .0234 \\ \midrule
\cmark &
  \cmark &
  \cmark &
  \cmark &
  9,232 &
  .0207 \\ \midrule
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Caption with \textless{}= 100 Words} (131,319 graph plots)} \\ \midrule
\multicolumn{2}{c}{\textbf{Subfig Filtering}} &
  \multicolumn{2}{c}{\textbf{Normalization}} &
   &
   \\ \cmidrule(r){1-4}
\textbf{Rule} &
  \textbf{FigSep} &
  \textbf{Basic} &
  \textbf{Adv} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Vocab\\ Size\end{tabular}}} &
  \multirow{-2}{*}{\textbf{BLEU-4}} \\ \midrule
 &
   &
   &
   &
  37,885 &
  .0231 \\ \midrule
\cmark &
   &
  \cmark &
   &
  30,316 &
  .0098 \\ \midrule
\cmark &
  \cmark &
  \cmark &
   &
  15,642 &
  .0173 \\ \midrule
\cmark &
  \cmark &
  \cmark &
  \cmark &
  14,974 &
  .0172 \\ \bottomrule
\end{tabular}
\caption{The baseline captioning model's performance on \dataset, using Vision-Only features.
Models trained on the first sentences of all the captions perform the best; normalizing caption improves the model's performance.
%; the text information (T) extracted from figures does not help the models. 
The low BLEU-4 scores indicate that more research is needed to generate caption for scientific figures reliably. 
%\kenneth{The vocab size is BEFORE pruning, right?}
(The vocabulary sizes were calculated after dropping words with a frequency less than five.)
%\cy{The dataset size would be different when applying different subfigure filtering methods right? Should we include those numbers?}\kenneth{You're right. Ed: is this true?}
\kenneth{Also, the 0.098 looks quite strange...}
}
\label{tab:text-only-result}
\end{table}

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/table.tex <==
\begin{table*}[h]
\footnotesize
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{Text Data} & Cleaning Method            & Text Normalization & Feature & Model          & BLEU-4 \\ \hline
1st Sent                        & None                       & None               & Vision  & CNN+LSTM       & 0.0131 \\ \hline
Single-Sent Caption             & None                       & None               & Vision  & CNN+LSTM       & 0.0115 \\ \hline
First 100 Words                 & None                       & None               & Vision  & CNN+LSTM       & 0.0091 \\ \hline
1st Sent                        & Rule-Based                 & Basic              & Vision  & CNN+LSTM       & 0.0202 \\ \hline
Single-Sent Caption             & Rule-Based                 & Basic              & Vision  & CNN+LSTM       & 0.0159 \\ \hline
First 100 Words                 & Rule-Based                 & Basic              & Vision  & CNN+LSTM       & 0.0141 \\ \hline
1st Sent                        & Rule-Based+FigureSeparator & Basic              & Vision  & CNN+LSTM       & 0.0366 \\ \hline
Single-Sent Caption             & Rule-Based+FigureSeparator & Basic              & Vision  & CNN+LSTM       & 0.0357 \\ \hline
First 100 Words                 & Rule-Based+FigureSeparator & Basic              & Vision  & CNN+LSTM       & 0.0318 \\ \hline
\textbf{1st Sent}                        & \textbf{Rule-Based+FigureSeparator} & \textbf{Basic + Advanced}   & \textbf{Vision}  & \textbf{CNN+LSTM}       & \textbf{0.0416} \\ \hline
Single-Sent Caption             & Rule-Based+FigureSeparator & Basic + Advanced   & Vision  & CNN+LSTM       & 0.0362 \\ \hline
First 100 Words                 & Rule-Based+FigureSeparator & Basic + Advanced   & Vision  & CNN+LSTM       & 0.0333 \\ \hline
Image Text                      & Rule-Based+FigureSeparator & Basic + Advanced   & Text    & LSTM (Seq2Seq) & 0.0203 \\ \hline
1st Sent                        & Rule-Based+FigureSeparator & Basic + Advanced   & V+T     & CNN+LSTM       & 0.0339 \\ \hline
Single-Sent Caption             & Rule-Based+FigureSeparator & Basic + Advanced   & V+T     & CNN+LSTM       & 0.0347 \\ \hline
First 100 Words                 & Rule-Based+FigureSeparator & Basic + Advanced   & V+T     & CNN+LSTM       & 0.0312 \\ \hline
\end{tabular}
%\caption{The baseline image captioning model's performance on \dataset. Models trained on the first sentences of all the captions perform the best; normalizing caption improves the model's performance; the text information (T) extracted from figures does not help the models. The low BLEU-4 scores indicate that more research is needed to generate caption for scientific figures reliably. \kenneth{1. Add more auto metrics, and (2) calculate the lexical diversity, e.g., mean segmental type-token ratio (MSTTR).}}
%\label{tab:baseline-results}
\end{table*}

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/tech-eval-table-graph-plot-only.tex <==


% 單一分類器的情況
% TN: 真多張 = (分類器說是多張, 實際上也是多張)  
% FN: 假多張 = (分類器說是多張, 實際上卻是單張)  
% TP: 真單張 = (分類器說是單張, 實際上也是單張)  
% FP: 假單張 = (分類器說是單張, 實際上卻是多張)

% 兩個分類器合起來的情況
% TN: 真多張 = (至少有一個分類器說是多張, 實際上也是多張)
% FN: 假多張 = (至少有一個分類器說是多張, 實際上卻是單張)  
% TP: 真單張 = (兩個分類器都說是單張, 實際上也是單張)  
% FP: 假單張 = (兩個分類器都說是單張, 實際上卻是多張)

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{@{}lrrrr@{}}
\toprule
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Figure Type Classification} (Class = Graph Plot)}  \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\textbf{Approach}          & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{Acc} \\ \midrule
\cite{siegel2016figureseer}              & .90        & .83        & .87        & .95          \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}\textbf{Non-Subfigure Figure Classification}\\ (For figures labeled as graph plots in Step 3.)\end{tabular}} \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\textbf{Approach}          & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{Acc} \\ \midrule
Rule-Based                 & .54        & .95        & .69        & .59          \\ \midrule
FigureSeparator            & .98        & .66       & .79        & .83          \\ \midrule
Rule-Based+FigureSeparator & .98        & .62        & .76        & .81          \\ \bottomrule
\end{tabular}
\caption{The tools used to construct \dataset evaluated on 1,926 labeled images.
For figure type classification, the overall performance over graph plots was reliable.
Regarding identifying the graph plots (as labeled automatically in Step 3) that do not contain subfigures, FigureSeparator achieved an exceptionally high precision.}
\label{tab:tech-eval}
\end{table}

%------------------- dead kitten --------

\begin{comment}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{@{}lrrrr@{}}
\toprule
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Figure Type Classification} (Class = Graph Plot)}     \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\textbf{Approach}           & \textbf{P}  & \textbf{R}  & \textbf{F} & \textbf{Acc} \\ \midrule
\cite{siegel2016figureseer}              & .90         & .83         & .87        & .95          \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Non-Subfigure Classification} (If labeled as Graph Plot in Step 3} \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\textbf{Approach}           & \textbf{P}  & \textbf{R}  & \textbf{F} & \textbf{Acc} \\ \midrule
Rule-Based Only                & .53         & .94         & .68        & .58          \\ \midrule
FigureSeparator Only             & .98         & .67        & .79        & .84          \\ \midrule
Rule-Based + FigureSeparator  & .98         & .63         & .77        & .82          \\ \bottomrule
\end{tabular}
%\vspace{-.5pc}
\caption{The tools used to construct \dataset evaluated on 1,926 labeled images.
For the figure type classification, the overall performance over graph plots was reliable.
Regarding identifying the graph plots that do not contain subfigures, FigureSeparator achieved an exceptionally high precision.}
\label{tab:tech-eval}
%\vspace{-1.2pc}
\end{table}


\end{comment}

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/tech-eval-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{@{}llrrrr@{}}
\toprule
\rowcolor[HTML]{EFEFEF} 
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Figure Type Classification}}                    \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\textbf{Approach}                 & \textbf{Fig. Type} & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{Acc} \\ \midrule
                                  & Graph Plot         & .90        & .83        & .87        & .95          \\ \cmidrule(l){2-6} 
\multirow{-2}{*}{Siegel {\em et al.}}   & Bar Chart          & .85        & .78        & .81        & .99          \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Subfigure Identification (Y/N)}}                          \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\textbf{Approach}                 & \textbf{Fig. Type} & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{Acc} \\ \midrule
                                  & Graph Plot         & .83        & .26        & .39        & .58          \\ \cmidrule(l){2-6} 
\multirow{-2}{*}{Rule-Based}      & Bar Chart          & 1.00        & .10        & .18        & .63          \\ \midrule
                                  & Graph Plot         & .77        & 0.99       & .86        & .84          \\ \cmidrule(l){2-6} 
\multirow{-2}{*}{FigureSeparator} & Bar Chart          & .EE        & .FF        & .GG        & .HH          \\ \midrule
                                  & Graph Plot         & .72        & .73        & .73        & .71          \\ \cmidrule(l){2-6} 
\multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Rule-Based +\\ FigureSeparator\end{tabular}} & Bar Chart & .MM & .NN & .OO & .PP \\ \bottomrule
\end{tabular}
\vspace{-.5pc}
\caption{The tools used to construct \dataset evaluated on 1,926 labeled images.
For the figure type classification,
the overall performance was reliable.
For the subfigure identification, the rule-based classifier yielded high precision but low recall; adding FigureSeparator improved performance.\kenneth{TODO: Fill out all the numbers! What is accuracy here?}\edward{wait for separator results}\kenneth{Oh so ADDING FigureSeparator decreased F1 score...?! What... Should we just use FigureSeparator by itself?}}
\label{tab:tech-eval}
\vspace{-1pc}
\end{table}

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/title.tex <==
\title{\dataset: Generating Captions for Scientific Figures}


%\newcommand{\kenneth}[1]{{\small\textcolor{blue}{\bf [#1 --Ken]}}}
%\newcommand{\edward}[1]{{\small\textcolor{red}{\bf [#1 --Ed]}}}
%\newcommand{\lee}[1]{{\small\textcolor{orange}{\bf [#1 --Lee]}}}
%\newcommand{\cy}[1]{{\small\textcolor{cyan}{\bf [#1 --CY]}}}

\newcommand{\kenneth}[1]{}
\newcommand{\edward}[1]{}
\newcommand{\lee}[1]{}
\newcommand{\cy}[1]{}

\newcommand{\dataset}{\textsc{SciCap}\xspace}

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/train_val_test_size.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{@{}llrr@{}}
\toprule
\textbf{Data Collection}      & \textbf{Train} & \textbf{Validate} &\textbf{Test} \\ 
\midrule
\multirow{2}{*}{First Sentence}      & xxx            & xxx.              & xxx          \\ 
\midrule{Single-Sent Caption} & xxx            & xxx.              & xxx          \\   
\midrule{Caption w/ \textless{}=100 words} & xxx            & xxx.              & xxx\\ \bottomrule
\end{tabular}
%\vspace{-.5pc}
\caption{The experimental results of models using Vision-Only, Text-Only, and Vision+Text features. Vision-Only and Text-Only features yielded similar performance. (All the subfigure-filtering and text-normalization steps were applied.)}
% The text extracted from figures did not help the models. 
% (All the subfigure-filtering and text-normalization steps were applied.)
%\edward{this set use the last one setting}}
\label{tab:text-and-vision-result}
%\cy{Do we have ``Vision Only'' and ``Text Only'' results for Single-Sentence and Caption with \textless{}= 100 Words?}
%\kenneth{This table needs to have 9 rows.}
%\vspace{-1pc}
\end{table}

==> EMNLP%202021%20(Figure%20Caption%2C%205%20pages%20%2B%20Ref%2C%20Due%20Sep%209)/v-and-t-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{@{}llr@{}}
\toprule
\textbf{Data Collection}                          & \textbf{Feature} & \textbf{BLEU-4} \\ \midrule
\multirow{3}{*}{First Sentence}                   & Vision Only      & .0219           \\ \cmidrule(l){2-3} 
                                                  & Vision+Text      & .0205           \\ \cmidrule(l){2-3} 
                                                  & Text Only        & .0213           \\ \midrule
\multirow{3}{*}{Single-Sent Caption}              & Vision Only      & .0207           \\ \cmidrule(l){2-3} 
                                                  & Vision+Text      & .0202           \\ \cmidrule(l){2-3} 
                                                  & Text Only        & .0212           \\ \midrule
\multirow{3}{*}{Caption w/ \textless{}=100 words} & Vision Only      & .0172           \\ \cmidrule(l){2-3} 
                                                  & Vision+Text      & .0168           \\ \cmidrule(l){2-3} 
                                                  & Text Only        & .0165           \\ \bottomrule
\end{tabular}
%\vspace{-.5pc}
\caption{The experimental results of models using Vision-Only, Text-Only, and Vision+Text features. Vision-Only and Text-Only features yielded similar performance. (All the subfigure-filtering and text-normalization steps were applied.)}
% The text extracted from figures did not help the models. 
% (All the subfigure-filtering and text-normalization steps were applied.)
%\edward{this set use the last one setting}}
\label{tab:text-and-vision-result}
%\cy{Do we have ``Vision Only'' and ``Text Only'' results for Single-Sentence and Caption with \textless{}= 100 Words?}
%\kenneth{This table needs to have 9 rows.}
%\vspace{-1pc}
\end{table}

==> baselines.tex <==
We use CNN + Long short-term memory(LSTM) structure as our baseline, which is typical architecture in Image Captioning task~\cite{xu2015show}. We extract the images features using the pre-trained  ResNet-101 model~\cite{he2016deep} and represent each figure a 2048-dimensional  vector. We then feed the vector into a dense layer to fit the dimension of word embedding and learn the adjusting transformation. 

==> old_emnlp_instruction.tex <==

These instructions are for authors submitting papers to EMNLP 2021 using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} as well as guidelines set forth in the EMNLP 2021 call for papers. This document contains additional instructions for the \LaTeX{} style files.

The templates include the \LaTeX{} source of this document (\texttt{emnlp2021.tex}),
the \LaTeX{} style file used to format it (\texttt{emnlp2021.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{emnlp2021}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{emnlp2021}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
\citealp{Gusfield:97} & \verb|\citealp| & no equivalent \\
\citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

% \nocite{Ando2005,borschinger-johnson-2011-particle,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{custom}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.



\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.


==> table-new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{@{}cccccc@{}}
\toprule
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{First Sentence} (133,543 graph plots)} \\ \midrule
\multicolumn{2}{c}{\textbf{Subfig Filtering}} &
  \multicolumn{2}{c}{\textbf{Normalization}} &
   &
   \\ \cmidrule(r){1-4}
\textbf{Rule} &
  \textbf{FigSep} &
  \textbf{Basic} &
  \textbf{Adv} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Vocab\\ Size\end{tabular}}} &
  \multirow{-2}{*}{\textbf{BLEU-4}} \\ \midrule
   &
   &
   &
   &
  30,776 &
  .0259 \\ \midrule
\cmark &
   &
  \cmark &
   &
  24,355 &
  .0236 \\ \midrule
\cmark &
  \cmark &
  \cmark &
   &
  12,666 &
  .0224 \\ \midrule
\cmark &
  \cmark &
  \cmark &
  \cmark &
  11,946 &
  .0219 \\ \midrule
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Single-Sentence Caption} (94,110 graph plots)} \\ \midrule
\multicolumn{2}{c}{\textbf{Subfig Filtering}} &
  \multicolumn{2}{c}{\textbf{Normalization}} &
   &
   \\ \cmidrule(r){1-4}
\textbf{Rule} &
  \textbf{FigSep} &
  \textbf{Basic} &
  \textbf{Adv} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Vocab\\ Size\end{tabular}}} &
  \multirow{-2}{*}{\textbf{BLEU-4}} \\ \midrule
 &
   &
   &
   &
  21,765 &
  .0291 \\ \midrule
\cmark &
   &
  \cmark &
   &
  17,685 &
  .0228 \\ \midrule
\cmark &
  \cmark &
  \cmark &
   &
  9,760 &
  .0234 \\ \midrule
\cmark &
  \cmark &
  \cmark &
  \cmark &
  9,232 &
  .0207 \\ \midrule
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Caption with \textless{}= 100 Words} (131,319 graph plots)} \\ \midrule
\multicolumn{2}{c}{\textbf{Subfig Filtering}} &
  \multicolumn{2}{c}{\textbf{Normalization}} &
   &
   \\ \cmidrule(r){1-4}
\textbf{Rule} &
  \textbf{FigSep} &
  \textbf{Basic} &
  \textbf{Adv} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Vocab\\ Size\end{tabular}}} &
  \multirow{-2}{*}{\textbf{BLEU-4}} \\ \midrule
 &
   &
   &
   &
  37,885 &
  .0231 \\ \midrule
\cmark &
   &
  \cmark &
   &
  30,316 &
  .0098 \\ \midrule
\cmark &
  \cmark &
  \cmark &
   &
  15,642 &
  .0173 \\ \midrule
\cmark &
  \cmark &
  \cmark &
  \cmark &
  14,974 &
  .0172 \\ \bottomrule
\end{tabular}
\caption{The baseline captioning model's performance on \dataset, using Vision-Only features.
Models trained on the first sentences of all the captions perform the best; normalizing caption improves the model's performance.
%; the text information (T) extracted from figures does not help the models. 
The low BLEU-4 scores indicate that more research is needed to generate caption for scientific figures reliably. 
%\kenneth{The vocab size is BEFORE pruning, right?}
(The vocabulary sizes were calculated after dropping words with a frequency less than five.)
%\cy{The dataset size would be different when applying different subfigure filtering methods right? Should we include those numbers?}\kenneth{You're right. Ed: is this true?}
\kenneth{Also, the 0.098 looks quite strange...}
}
\label{tab:text-only-result}
\end{table}

==> table.tex <==
\begin{table*}[h]
\footnotesize
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{Text Data} & Cleaning Method            & Text Normalization & Feature & Model          & BLEU-4 \\ \hline
1st Sent                        & None                       & None               & Vision  & CNN+LSTM       & 0.0131 \\ \hline
Single-Sent Caption             & None                       & None               & Vision  & CNN+LSTM       & 0.0115 \\ \hline
First 100 Words                 & None                       & None               & Vision  & CNN+LSTM       & 0.0091 \\ \hline
1st Sent                        & Rule-Based                 & Basic              & Vision  & CNN+LSTM       & 0.0202 \\ \hline
Single-Sent Caption             & Rule-Based                 & Basic              & Vision  & CNN+LSTM       & 0.0159 \\ \hline
First 100 Words                 & Rule-Based                 & Basic              & Vision  & CNN+LSTM       & 0.0141 \\ \hline
1st Sent                        & Rule-Based+FigureSeparator & Basic              & Vision  & CNN+LSTM       & 0.0366 \\ \hline
Single-Sent Caption             & Rule-Based+FigureSeparator & Basic              & Vision  & CNN+LSTM       & 0.0357 \\ \hline
First 100 Words                 & Rule-Based+FigureSeparator & Basic              & Vision  & CNN+LSTM       & 0.0318 \\ \hline
\textbf{1st Sent}                        & \textbf{Rule-Based+FigureSeparator} & \textbf{Basic + Advanced}   & \textbf{Vision}  & \textbf{CNN+LSTM}       & \textbf{0.0416} \\ \hline
Single-Sent Caption             & Rule-Based+FigureSeparator & Basic + Advanced   & Vision  & CNN+LSTM       & 0.0362 \\ \hline
First 100 Words                 & Rule-Based+FigureSeparator & Basic + Advanced   & Vision  & CNN+LSTM       & 0.0333 \\ \hline
Image Text                      & Rule-Based+FigureSeparator & Basic + Advanced   & Text    & LSTM (Seq2Seq) & 0.0203 \\ \hline
1st Sent                        & Rule-Based+FigureSeparator & Basic + Advanced   & V+T     & CNN+LSTM       & 0.0339 \\ \hline
Single-Sent Caption             & Rule-Based+FigureSeparator & Basic + Advanced   & V+T     & CNN+LSTM       & 0.0347 \\ \hline
First 100 Words                 & Rule-Based+FigureSeparator & Basic + Advanced   & V+T     & CNN+LSTM       & 0.0312 \\ \hline
\end{tabular}
%\caption{The baseline image captioning model's performance on \dataset. Models trained on the first sentences of all the captions perform the best; normalizing caption improves the model's performance; the text information (T) extracted from figures does not help the models. The low BLEU-4 scores indicate that more research is needed to generate caption for scientific figures reliably. \kenneth{1. Add more auto metrics, and (2) calculate the lexical diversity, e.g., mean segmental type-token ratio (MSTTR).}}
%\label{tab:baseline-results}
\end{table*}

==> tech-eval-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{@{}llrrrr@{}}
\toprule
\rowcolor[HTML]{EFEFEF} 
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Figure Type Classification}}                    \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\textbf{Approach}                 & \textbf{Fig. Type} & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{Acc} \\ \midrule
                                  & Graph Plot         & .90        & .83        & .87        & .95          \\ \cmidrule(l){2-6} 
\multirow{-2}{*}{Siegel {\em et al.}}   & Bar Chart          & .85        & .78        & .81        & .99          \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Subfigure Identification (Y/N)}}                          \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\textbf{Approach}                 & \textbf{Fig. Type} & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{Acc} \\ \midrule
                                  & Graph Plot         & .83        & .26        & .39        & .58          \\ \cmidrule(l){2-6} 
\multirow{-2}{*}{Rule-Based}      & Bar Chart          & 1.00        & .10        & .18        & .63          \\ \midrule
                                  & Graph Plot         & .77        & 0.99       & .86        & .84          \\ \cmidrule(l){2-6} 
\multirow{-2}{*}{FigureSeparator} & Bar Chart          & .EE        & .FF        & .GG        & .HH          \\ \midrule
                                  & Graph Plot         & .72        & .73        & .73        & .71          \\ \cmidrule(l){2-6} 
\multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Rule-Based +\\ FigureSeparator\end{tabular}} & Bar Chart & .MM & .NN & .OO & .PP \\ \bottomrule
\end{tabular}
\vspace{-.5pc}
\caption{The tools used to construct \dataset evaluated on 1,926 labeled images.
For the figure type classification,
the overall performance was reliable.
For the subfigure identification, the rule-based classifier yielded high precision but low recall; adding FigureSeparator improved performance.\kenneth{TODO: Fill out all the numbers! What is accuracy here?}\edward{wait for separator results}\kenneth{Oh so ADDING FigureSeparator decreased F1 score...?! What... Should we just use FigureSeparator by itself?}}
\label{tab:tech-eval}
\vspace{-1pc}
\end{table}

==> train_val_test_size.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{@{}llrr@{}}
\toprule
\textbf{Data Collection}      & \textbf{Train} & \textbf{Validate} &\textbf{Test} \\ 
\midrule
\multirow{2}{*}{First Sentence}      & xxx            & xxx.              & xxx          \\ 
\midrule{Single-Sent Caption} & xxx            & xxx.              & xxx          \\   
\midrule{Caption w/ \textless{}=100 words} & xxx            & xxx.              & xxx\\ \bottomrule
\end{tabular}
%\vspace{-.5pc}
\caption{The experimental results of models using Vision-Only, Text-Only, and Vision+Text features. Vision-Only and Text-Only features yielded similar performance. (All the subfigure-filtering and text-normalization steps were applied.)}
% The text extracted from figures did not help the models. 
% (All the subfigure-filtering and text-normalization steps were applied.)
%\edward{this set use the last one setting}}
\label{tab:text-and-vision-result}
%\cy{Do we have ``Vision Only'' and ``Text Only'' results for Single-Sentence and Caption with \textless{}= 100 Words?}
%\kenneth{This table needs to have 9 rows.}
%\vspace{-1pc}
\end{table}
